PPO-ABR: Proximal Policy Optimization based Deep Reinforcement Learning for Adaptive BitRate streaming

Providing a high Quality of Experience (QoE) for video streaming in 5G and beyond 5G (B5G) networks is challenging due to the dynamic nature of the underlying network conditions. Several Adaptive Bit Rate (ABR) algorithms have been developed to improve QoE, but most of them are designed based on fixed rules and unsuitable for a wide range of network conditions. Recently, Deep Reinforcement Learning (DRL) based Asynchronous Advantage Actor-Critic (A3C) methods have recently demonstrated promise in their ability to generalise to diverse network conditions, but they still have limitations. One specific issue with A3C methods is the lag between each actor's behavior policy and central learner's target policy. Consequently, suboptimal updates emerge when the behavior and target policies become out of synchronization. In this paper, we address the problems faced by vanilla-A3C by integrating the on-policy-based multi-agent DRL method into the existing video streaming framework. Specifically, we propose a novel system for ABR generation - Proximal Policy Optimization-based DRL for Adaptive Bit Rate streaming (PPO-ABR). Our proposed method improves the overall video QoE by maximizing sample efficiency using a clipped probability ratio between the new and the old policies on multiple epochs of minibatch updates. The experiments on real network traces demonstrate that PPO-ABR outperforms state-of-the-art methods for different QoE variants.

==> sections/relatedwork.tex <==
\section{Related Work}\label{section:relatedwork}
%Several researchers have previously focused on designing ABR algorithms to increase
%QoE for video streaming, with the algorithms being constructed using preset criteria. Some of the fixed control rule based ABR algorithms include FESTIVE\cite{festive}, RB\cite{rb}, BB\cite{bb}, BOLA\cite{bola} and DYNAMIC\cite{dynamic}. These algorithms make decisions based on either the current buffer size or the estimated throughput. Moreover,  model predictive control (MPC) \cite{mpc} makes use of both buffer size and throughput prediction to make ABR decisions.

Due to the limited capability of fixed rule-based algorithms, recent studies are focused on machine learning-based hybrid control ABR algorithms, specifically focusing on the RL-based A3C \cite{a3c} methods. Such algorithms include Pensieve \cite{pensieve}, NANCY \cite{nancy}, SAC-ABR \cite{SAC-ABR}, AL-FFEA3C \cite{journal}, AL-AvgA3C \cite{journal}, MARL-A3C \cite{marl}, and deep Q-learning algorithm \cite{dqn} in HD3 \cite{hd3}. Benefiting from the capabilities of neural networks for feature extraction and policy learning, these algorithms obtain a balance between exploration and exploitation, less variance, maximize the QoE with more exploration, tackle the issue with overestimation of q-value using the double Q technique, and  outperform the fixed-rule based ABR algorithms over different variants of QoE metrics. However, most of the above-cited methods use both on-policy and off-policy A3C methods \cite{a3c}. Some other examples of off-policy-based RL algorithms also include TRPO \cite{trpo} and PPO\cite{ppo}. 

Our main contribution is to integrate the A3C gradient sharing on-policy algorithm in video streaming delivery over the existing A3C on-policy method for the following reasons: (i) requires small learning rates and lower entropy loss weights,
(ii) requires few numbers of workers with faster convergence,
(iii) high cumulative rewards with more exploration,
(iv) reduces the biases by more exploration at the initial stages and slowly converges to the optimal policy.



